GAAMA 2.0: An Integrated System that Answers Boolean and Extractive Questions

Recent machine reading comprehension datasets include extractive and boolean questions but current approaches do not offer integrated support for answering both question types. We present a multilingual machine reading comprehension system and front-end demo that handles boolean questions by providing both a YES/NO answer and highlighting supporting evidence, and handles extractive questions by highlighting the answer in the passage. Our system, GAAMA 2.0, is ranked first on the Tydi QA leaderboard at the time of this writing. We contrast two different implementations of our approach. The first includes several independent stacks of transformers allowing easy deployment of each component. The second is a single stack of transformers utilizing adapters to reduce GPU memory footprint in a resource-constrained environment.

==> data.tex <==
\section{Data}

\begin{table}[t]
%\small
\centering
    \begin{tabular}{l|l|l|} %{\columnwidth}
%    \toprule
     \textbf{Dataset} & \textbf{Train} &\textbf{Dev} \\
     \hline
%     \midrule
     TyDi & 562 & 78 \\
     BoolQ & NA & 2063 + 315 \\
%     \bottomrule
    \end{tabular}
    \caption{Number of Boolean instances in the TyDi English and BoolQ datasets annotated for evidence.}
    \label{tab:data-stats}
\end{table}

We use two datasets that contain Boolean Questions in our analysis and experiments: TyDi \cite{clark-etal-2020-tydi} and BoolQ \cite{clark-etal-2019-boolq}.

\subsection{\tydi}

\tydi is an Multilingual MRC dataset containing questions in multiple languages. 10\% of the data is Boolean Questions. The TyDi boolean questions annotations include the paragraph the answer is found in and a label: YES or NO. A boolean question can also be unanswerable. It is important to note that there is an extreme skew towards the answers being YES at 80\%, meaning that the ability of the evidence classifier to correctly predict NO has limited impact upon end-to-end Tydi results.

\subsection{Expanded BoolQ}

BoolQ is large datasets consisting of over 18k naturally occurring Boolean questions.
There are two limitations of the BoolQ dataset that limit its applicability to our scenario. 
All of the questions have answers in the given passage.
Also the passages are very short, averaging about 100 words each.

In order to make the BoolQ data more similar to the \tydi data, we locate (by title) the source Wikipedia article for each BoolQ passage in the 2018-12-20 Wikipedia dump.
(Note that the original BoolQ passages had been retrieved from the "live" Wikipedia.)
We extract 200 and 500 word passages from the wikipedia article centered on the original BoolQ passage.
We also extract another 200 word passage, chosen {\em not} to overlap with the original BoolQ passage as pseudo-no-answer sample.
We use the 200 word passages, both as additional training data, and as an additional dev set for development of the evidence classifier.
We use the 500 word passages as an additional end-to-end test of the GAAMA system.

%This mismatch in Wikipedia versions caused a loss of some questions in the original dataset from 3.2k to 2.4k dev instances.




%Because of the limitations of the Tydi dataset, we also leverage the BoolQ dataset, but in a non-traditional manner.

%BoolQ provides the question, Boolean answer as YES or NO, and a short passage of around 100. 
%To obtain reliable evidence we expand the passage to the surrounding 200 words. We created this using Wikipedia dump XX (Wikipedia dump used in BoolQ is unknown) which caused a loss of some questions in the original dataset from 3.2k to 2.5k dev instances, of which 315 questions were found to have be unanswerable by our annotators.



==> evc_results_accuracy.tex <==
\begin{table*}[hbt!]
    \centering
    % \small
    \begin{tabular}{c|c||c|c||c}
         \textbf{system} & \textbf{spans} &\textbf{TydiDev (ternary)} &
         \textbf{TydiDev (binary)} &
         \textbf{BoolQ-X Dev} \\
	\hline
%BPES (spans) & gold & 60.1 & 82.6 & 75.1 \\
%BPES (spans) & sys & 63.6 & 81.7 & 74.6 \\
%BPES (passages) & gold	&	52.6	&	84.6 & 75.4	\\
BPES (passages) & sys	&	71.0	&	81.9 & 73.5\\
\hline
adapter(OOB) (passage) & sys & 71.4 & 81.7 & 74.0 \\
adapter(MRC) (passage) & sys & 72.1 & 83.1 & 76.3 \\
\hline
%xlmr(tydi-mrc)+adapters & gold & 85.5 & 76.8 \\
%xlmr(tydi-mrc)+adapters & sys & 84.3 & 76.3 \\
%xlmr(oob)+adapters & gold & 86.1 & 74.2 \\
%xlmr(oob)+adapters & sys & 84.3 & 74.0 \\
    \end{tabular}
    \caption{Evidence Span classifier results.  TydiDev.  BoolQ is 3-way classification accuracy}
    \label{tab:evc-results}
\end{table*}

==> evc_results_adapter.tex <==
% these use the original qtc to generate the dev set
\begin{table}[t]
\small
\begin{center}
%\begin{tabular}{|l|l||c|c|c|c|c||c|c|c|c|c|}
\begin{tabular}{|l|l||c|c||c|c|}
\toprule
\multirowthead{2}{model} &
\multirowthead{2}{unit} &
%\multicolumn{3}{c|}{\tydi{}} & 
\multicolumn{2}{c||}{BoolQ-X} &
%\multicolumn{3}{c|}{BoolQ-X} & 
\multicolumn{2}{c|}{\tydi{} } \\ 
%\cline{3-5} \cline{6-7} \cline{8-10} \cline{11-12}
&
%& No & NA & Yes
& NO & YES
%& No & NA & Yes
& NO & YES \\


\midrule
%$ \hbox{bpes (sys)}    $ & span 
%& 59.3 & 82.2 & 72.9 
%& 66.3 & 81.8
%& 30.0 & 67.9 & 65.1
%& 35.7 & 89.3 \\
$ \hbox{bpes (sys)} $ & passage
%& 58.7 & 82.0 & 72.1
& 65.7 & 81.3
%& 33.6 & 77.4 & 70.4
& 44.5 & 91.0 \\
%$ \hbox{adapter (oob)} $ & passage
%& 60.0 & 82.2 & 72.6 
%& 66.5 & 81.4 
%& 31.1 & 77.7 & 71.5
%& 46.7 & 90.8 \\
$ \hbox{adapter (mrc)} $ & passage 
%& 62.6 & 84.1 & 75.0 
& 68.8 & 83.0
%& 35.8 & 77.0 & 72.6
& 41.5 & 90.9 \\
\bottomrule
\end{tabular}
\end{center}
\caption{Evidence Span classifier results.}  
\label{tab:evc-results_adapter}
\end{table}


==> evc_results_binary.tex <==
% these use the mrc-adapter qtc to generate the dev set

\begin{table*}
\small
\begin{center}
%\begin{tabular}{|l|l||c|c|c|c|c||c|c|c|c|c|}
\begin{tabular}{|l|l||c|c||c|c|}
\toprule
\multirowthead{2}{model} &
\multirowthead{2}{unit} &
%\multicolumn{3}{c|}{\tydi{}} & 
\multicolumn{2}{c||}{BoolQ-X} &
%\multicolumn{3}{c|}{BoolQ-X} & 
\multicolumn{2}{c|}{\tydi{} } \\ 
%\cline{3-5} \cline{6-7} \cline{8-10} \cline{11-12}
&
%& No & NA & Yes
& No & Yes
%& No & NA & Yes
& No & Yes \\


\midrule
$ \hbox{bpes (sys)}    $ & span 
%& 59.3 & 82.2 & 72.9 
& 66.3 & 81.8
%& 30.0 & 67.9 & 65.1
& 35.7 & 89.3 \\
$ \hbox{bpes (sys)} $ & passage
%& 58.7 & 82.0 & 72.1
& 65.7 & 81.3
%& 33.6 & 77.4 & 70.4
& 39.0 & 89.4 \\
$ \hbox{adapter (oob)} $ & passage
%& 60.0 & 82.2 & 72.6 
& 66.5 & 81.4 
%& 31.1 & 77.7 & 71.5
& 39.7 & 89.2 \\
$ \hbox{adapter (mrc)} $ & passage 
%& 62.6 & 84.1 & 75.0 
& 68.8 & 83.0
%& 35.8 & 77.0 & 72.6
& 42.5 & 90.1 \\
\bottomrule
\end{tabular}
\end{center}
\caption{Evidence Span classifier results.}  
\label{tab:evc-results2-mrcadapt}
\end{table*}





==> evc_results_binary2.tex <==
% these use the original qtc to generate the dev set
\begin{table*}[ht]
\small
\begin{center}
%\begin{tabular}{|l|l||c|c|c|c|c||c|c|c|c|c|}
\begin{tabular}{|l|l||c|c||c|c|}
\toprule
\multirowthead{2}{model} &
\multirowthead{2}{unit} &
%\multicolumn{3}{c|}{\tydi{}} & 
\multicolumn{2}{c||}{BoolQ-X} &
%\multicolumn{3}{c|}{BoolQ-X} & 
\multicolumn{2}{c|}{\tydi{} } \\ 
%\cline{3-5} \cline{6-7} \cline{8-10} \cline{11-12}
&
%& No & NA & Yes
& No & Yes
%& No & NA & Yes
& No & Yes \\


\midrule
$ \hbox{bpes (sys)}    $ & span 
%& 59.3 & 82.2 & 72.9 
& 66.3 & 81.8
%& 30.0 & 67.9 & 65.1
& 35.7 & 89.3 \\
$ \hbox{bpes (sys)} $ & passage
%& 58.7 & 82.0 & 72.1
& 65.7 & 81.3
%& 33.6 & 77.4 & 70.4
& 44.5 & 91.0 \\
%$ \hbox{adapter (oob)} $ & passage
%& 60.0 & 82.2 & 72.6 
%& 66.5 & 81.4 
%& 31.1 & 77.7 & 71.5
%& 46.7 & 90.8 \\
%$ \hbox{adapter (mrc)} $ & passage 
%& 62.6 & 84.1 & 75.0 
%& 68.8 & 83.0
%& 35.8 & 77.0 & 72.6
%& 41.5 & 90.9 \\
\bottomrule
\end{tabular}
\end{center}
\caption{Evidence Span classifier results.}  
\label{tab:evc-results2-orig}
\end{table*}





==> evc_results_f1all.tex <==
\begin{table*}
\small
\begin{center}
\begin{tabular}{|l|l||c|c|c|c|c||c|c|c|c|c|}
\toprule
\multirowthead{2}{model} &
\multirowthead{2}{unit} &
\multicolumn{3}{c|}{\tydi{}} & 
\multicolumn{2}{c||}{\tydi{} (2)} &
\multicolumn{3}{c|}{BoolQ-X} & 
\multicolumn{2}{c|}{BoolQ-X (2)} \\
%\cline{3-5} \cline{6-7} \cline{8-10} \cline{11-12}
& & No & NA & Yes & No & Yes & No & NA & Yes & No & Yes \\


\midrule
$ \hbox{bpes (sys)}    $ & span 
& 59.3 & 82.2 & 72.9 
& 66.3 & 81.8
& 30.0 & 67.9 & 65.1
& 35.7 & 89.3 \\
$ \hbox{bpes (sys)} $ & passage
& 58.7 & 82.0 & 72.1
& 65.7 & 81.3
& 33.6 & 77.4 & 70.4
& 39.0 & 89.4 \\
$ \hbox{adapter (oob)} $ & passage
& 60.0 & 82.2 & 72.6 
& 66.5 & 81.4 
& 31.1 & 77.7 & 71.5
& 39.7 & 89.2 \\
$ \hbox{adapter (mrc)} $ & passage 
& 62.6 & 84.1 & 75.0 
& 68.8 & 83.0
& 35.8 & 77.0 & 72.6
& 42.5 & 90.1 \\
\bottomrule
\end{tabular}
\end{center}
\caption{Evidence Span classifier results.  TydiDev.  BoolQ is 3-way classification accuracy}
\label{tab:evc-results2}
\end{table*}


==> evc_results_ternary.tex <==
\begin{table*}
\small
\begin{center}
%\begin{tabular}{|l|l||c|c|c|c|c||c|c|c|c|c|}
\begin{tabular}{|l|l||c|c|c||c|c|c|}
\toprule
\multirowthead{2}{model} &
\multirowthead{2}{unit} &
\multicolumn{3}{c||}{\tydi{}} & 
%\multicolumn{2}{c||}{\tydi{} (2)} &
\multicolumn{3}{c|}{BoolQ-X}  \\
%\multicolumn{2}{c|}{BoolQ-X (2)} \\ 
%\cline{3-5} \cline{6-7} \cline{8-10} \cline{11-12}
&
& No & NA & Yes
% & No & Yes
& No & NA & Yes
% & No & Yes
\\


\midrule
$ \hbox{bpes (sys)}    $ & span 
& 59.3 & 82.2 & 72.9 
%& 66.3 & 81.8
& 30.0 & 67.9 & 65.1
%& 35.7 & 89.3
\\
$ \hbox{bpes (sys)} $ & passage
& 58.7 & 82.0 & 72.1
%& 65.7 & 81.3
& 33.6 & 77.4 & 70.4
%& 39.0 & 89.4
\\
$ \hbox{adapter (oob)} $ & passage
& 60.0 & 82.2 & 72.6 
%& 66.5 & 81.4 
& 31.1 & 77.7 & 71.5
%& 39.7 & 89.2
\\
$ \hbox{adapter (mrc)} $ & passage 
& 62.6 & 84.1 & 75.0 
%& 68.8 & 83.0
& 35.8 & 77.0 & 72.6
%& 42.5 & 90.1
\\
\bottomrule
\end{tabular}
\end{center}
\caption{Evidence Span classifier results.  TydiDev.  BoolQ is 3-way classification accuracy}
\label{tab:evc-results2}
\end{table*}



==> experiments.tex <==
\section{Experiments}

In this section we present both end-to-end results of our system on half of the Tydi dev set, and performance of individual components on the same half of the Tydi and the extended version of BoolQ.
We used files 5-9 of the Tydi dev set because files 0-4 were used in calibrating the score normalization component.
We further compare the performance of components as implemented using independent stacks of transformers with component implementations using adapters.
All experiments were implemented using the frameworks from \cite{wolf-etal-2020-transformers}
and \cite{pfeiffer2020AdapterHub}.

In order to make the BoolQ data more similar to the \tydi data, we locate (by title) the source Wikipedia article for each BoolQ passage in the 2018-12-20 Wikipedia dump.
(Note that the original BoolQ passages had been retrieved from the "live" Wikipedia.)
We extract 200 and 500 word passages from the wikipedia article centered on the original BoolQ passage.
We also extract another 200 word passage, chosen {\em not} to overlap with the original BoolQ passage as pseudo-no-answer sample.
We use the 200 word passages, both as additional training data, and as an additional dev set for development of the evidence classifier.
We use the 500 word passages as an additional end-to-end test of the GAAMA system.


\begin{table}[hbt!]
\centering
\begin{tabular}{|c|c|c|}
\textbf{system} & \textbf{Split} & \textbf{SA}  \\
\hline
%\hbox{BASE}            &   69.3 & 73.7 \\
%\hbox{BASE+QTC\_SN+YES} &  72.2 & 73.7 \\
%\hbox{BASE+QTC\_SN+ESC} &  72.2 & 73.7 \\
%\hline
\hbox{BPES}            & Dev & 68.6\\
\hbox{BPES+QTC\_SN+YES} & Dev &  72.5  \\
\hbox{BPES+QTC\_SN+ESC} & Dev &  72.6 & 74.8 \\
\hline
\hbox{GAAMA-Syn-Bool-Single-Model} & Test  & 72.35 \\
\hbox{GAAMA-DM-Syn-ARES} & Test & 68.06  \\
\hbox{PoolingFormer} & Test & 67.65  \\
\hline
\end{tabular}
\caption{ End-to-End Results on half of the Tydi dev set and TyDi test set.  Test set results are evaluated by the TyDi QA leaderbord 
%Tydi dev set was used in training the score normalizer and/or the evidence span classifier
}
\label{tab:tydi-results}
\end{table}



\subsection{Tydi results}
In Table \ref{tab:tydi-results}, we show short-answer (SA) and passage answer (SA) tydi results on half of the Tydi dev set.
BASE is a baseline xlm-roberta system trained on the Tydi data, with no special treatment of the boolean questions.  In BASE+QTC\_SN+YES, we include a query type classifier to identify the boolean questions, the score normalization component to identify answerable questions, and (taking advantage of the skew in Tydi data) we provide an answer of YES to those questions automatically identified as boolean.
This is the clearest demonstration of the value of the score normalization component - it is an enabling component that is necessary for demonstrating the value of the query type classifier.
In BASE+QTC\_SN+ESC, the evidence classifier is added.
Unfortunately because of the high baseline (few of the answer Tydi boolean questions are NO) no additional improvement is seen here.

In BPSE, the MRC classifier is additionally provided with the passage answer for the boolean questions (the dataset does not provide a short answer).  
This does not show an improvement over BASE, until the additional components for treating boolean questions are added.
These results are on half of the dev set of Tydi.  They are validated by the top-ranked performance of our GAAMA system (identical to BPES+QTC\_SN+ESC) on the hidden test set of the Minimal Answer Task of the Tydi leaderboard.
\footnote{https://ai.google.com/research/tydiqa, retrieved 2022-01-12}

\begin{table}[t]
%\small
\centering
    \begin{tabular}{l|l|l|} %{\columnwidth}
%    \toprule
     \textbf{model} & \textbf{factoid} &\textbf{boolean} \\
     \hline
%     \midrule
     mBERT & 99.2 & 94.6 \\
     tydi-mrc(xlmr)+adapters & 99.6 & 97.3 \\
%     \bottomrule
    \end{tabular}
    \caption{Classification of questions into boolean/factoid in TyDi (all languages)}
    \label{tab:qtype_results}
\end{table}


\subsection{Query Type Classifier}
The query type classifier was evaluated on the answerable subset of the Tydi questions.
(The NO-ANSWER tydi questions were not labeled as boolean or non-boolean.)
We compared a baseline transformer model with an adapter based model in which the adapter is applied directly to trained span selection model, in order to leverage its additional training data.
We find Table \ref{tab:qtype_results} that performance actually improved with the use of the adapter compared to the component in our leaderboard submission.

%\input{evc_results_accuracy}

%\input{evc_results_f1all}
\input{evc_results_binary}
\input{evc_results_ternary}




\subsection{Evidence classifier results}

In Table \ref{tab:evc-results}, we show evidence classifier accuracies on half of the Tydi development set, and on the expanded Boolq dev set.  
For Tydi, these results are only on those questions that are automatically determined to be boolean by the query type classifier.
Note that these questions may have answer of YES, NO, or NONE.  We report results on both the ternary classification task, and on the binary classification task of predicting YES or NO on those questions that are answerable in the gold dataset.

For much of system development we relied on TydiDev (ternary) comparisons.  The TydiDev (binary) subset was found to be highly skewed, and did not provide sufficient resolution to inform decisions, other than as a final sanity check.  We also validated our results on the BoolQ-X dev set.

\subsubsection{gold vs system training}
We see in Table \ref{tab:evc-results} that training with system spans generally outperformed training with gold spans. 
The system spans were obtained by 6-fold cross-validation in the Tydi training set.
Since the evidence classifier operates on system output, training on matched conditions is a appropriate design choice.

\subsubsection{passages vs. spans}
We compared building the evidence classifier on the output spans of the MRC system, versus expanding the spans to the containing paragraph boundaries (provided in the Tydi data). The expansion seems to help with system training (our use case), but did not help the system trained with gold passages.  Note that this is a very data-specific heuristic - on a real system we simply expand the system-generated spans into wider windows based on fixed offsets to the begin and end of the spans.

\subsection{Adapters vs. Independent transformers}

We compare an evidence classifier fine-tuned independently from the other components with two different adapter-based implementations.
In adapter(OOB), which applies the adapter directly to the standard xlm-roberta, we see that the overall performance is comparable to the performance of BPES(passages), which is encouraging.
In adapter(MRC), the adapter is applied directly to the trained span selection model.  This allows the evidence classifier to leverage the additional training data seen by the MRC model.  We see an encouraging improvement in performance across all three accuracy measurements.



















%\begin{figure}
%  \centering
%  \includegraphics[width=1\linewidth]{score_histogram.png}
%   \caption{score histogram}
%   \label{fig:score_histogram}
%\end{figure}


\FloatBarrier
